Millimeter Wave Full-Duplex Radios: New Challenges and Techniques

Equipping millimeter wave (mmWave) systems with full-duplex capability would accelerate and transform next-generation wireless applications and forge a path for new ones. Full-duplex mmWave transceivers could capitalize on the already attractive features of mmWave communication by supplying spectral efficiency gains and latency improvements while also affording future networks with deployment solutions in the form of interference management and wireless backhaul. Foreseeable challenges and obstacles in making mmWave full-duplex a reality are presented in this article along with noteworthy unknowns warranting further investigation. With these novelties of mmWave full-duplex in mind, we lay out potential solutions---beyond active self-interference cancellation---that harness the spatial degrees of freedom bestowed by dense antenna arrays to enable simultaneous transmission and reception in-band.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> sec-keywords.tex <==
\begin{keywords}
Millimeter-wave
\end{keywords}

==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle

==> sec-response.tex <==
\section*{Response to Reviewers}

\subsection*{Editor, Guest Editors, and Reviewers 1, 2, 3, and 4}

Thank you for carefully reading our paper and providing helpful comments and suggestions that have led to the enclosed revision. 
We have detailed the actions taken in response to your suggestions below. 
Your comments are in \textit{italics} with our response in plaintext.

\vspace{0.5cm}

\noindent Sincerely,\\
Ian P. Roberts\\
Jeffrey G. Andrews\\
Hardik B. Jain\\
Sriram Vishwanath\\


\subsection*{Reviewer 1}


\textit{This paper investigates millimeter-wave full-duplex communications, where the challenges and obstacles are presented and potential solutions are discussed. I have some major concerns as follows:}

\textit{1. Some important works on mmWave full-duplex communications are missing.}
\begin{itemize}
\item {[R1]}: Full-Duplex Millimeter-Wave Communication, IEEE Wireless Communications 2017.
\item {[R2]}: Millimeter-Wave Full-Duplex UAV Relay: Joint Positioning, Beamforming, and Power Control, IEEE JSAC 2020.
\end{itemize}

The two papers are very related to the topic of this paper. Especially in [R1], a similar tutorial has been studied on mmWave full-duplex systems, including the antenna structure, channel modeling, beamforming-aided self-interference cancelation, etc. The authors are suggested to show the main differences between this paper and the existing works and make the contribution of this paper clearer.



2. In the fifth paragraph of Section II, the authors should provide more explanations on how these components (PA, LNA, DAC, ADC) impact the mmWave full-duplex systems compared to the half-duplex or general communication systems.

We agree there is not much in-depth discussion of these crucial components. For the scope of this paper, given that mmWave full-duplex is in its infancy, we felt the most important difference between sub-6 GHz and mmWave full-duplex in this regard is the sheer number of PAs and LNAs and their placement. This fact is particularly important in two regards: (1) justifying why analog SIC doesn't seem practical and (2) pointing out the need to avoid LNA and ADC saturation. Beyond this, we have tried to sprinkle in small remarks regarding ADC resolution and self-interference, PA nonlinearity, and how such wideband communication at mmWave may make frequency-selectivity and nonlinearity more pronounced. We hope readers interested in these topics can find nuggets of inspiration for future work in our article. We think a thorough investigation of transceiver nonlinearity would offer valuable insights.

In light of your feedback, we have revised and added a few remarks on the impacts of transceiver components in mmWave full-duplex:
The last paragraph of Section II: The Implications of Hybrid Beamforming Architectures
Fortunately, digital SIC remains a promising candidate for mmWave full-duplex since the number of RF chains remains low with hybrid beamforming, though exaggerated impairments in mmWave transceivers may drive up computational costs if not dealt with beforehand. A deeper investigation into digital SIC for mmWave full-duplex would likely yield many useful insights, particularly on transceiver nonlinearity and other impairments such as I/Q imbalance, carrier frequency offset, and phase noise making it a good topic for future work.
Importantly, understanding how beamforming cancellation interacts with nonlinear terms induced by the transmit PAs will shed light on the system design of mmWave full-duplex.



3. In Section V, a nonrepresentational analysis is provided to show the basic intertwining of the transmitter and receiver beamforming. The authors are suggested to provide an overview on the state-of-the-art and real-world solutions of beamforming-aided SIC in mmWave full-duplex systems, such as [R2], [9], [12].

We certainly would like to overview existing beamforming cancellation designs in this article, but we felt it may not be a good use of space given the length constraint of this article. Instead, we felt presenting a more abstract and universal depiction of beamforming cancellation and how it can resemble familiar zero-forcing and MMSE approaches may be more likely to foster future research. Of course, we have included a few references including [9] and [12] with the hope that interested readers can investigate the details of these existing works as desired. Currently, we are not familiar with anything regarding real-world beamforming-based solutions for mmWave full-duplex.

4. The conclusion section should be strengthened to provide the readers with more knowledge and inspiration for future research.

